Characterizing the Accuracy -- Efficiency Trade-off of Low-rank Decomposition in Language Models

Recent large language models (LLMs) employ billions of parameters to enable broad problem-solving capabilities. Such language models also tend to be memory-bound because of the dominance of matrix-vector and matrix-matrix multiplications with low arithmetic intensity. Therefore, optimizing the memory footprint and traffic is an important optimization direction for LLMs today. Model compression methods such as quantization and parameter pruning have been actively explored to achieve memory footprint and traffic optimization. However, the accuracy-efficiency trade-off of rank pruning (i.e., low-rank decomposition) for LLMs is not well-understood yet. Therefore, in this work, we characterize the accuracy-efficiency trade-off of a low-rank decomposition method, specifically Tucker decomposition, on recent language models, including an open-source LLM, Llama 2. We formalize the low-rank decomposition design space and show that the decomposition design space is enormous (e.g., O($2^{39}$) for Llama2-7B). To navigate such a vast design space, we formulate it and perform thorough case studies of accuracy-efficiency trade-offs using six widely used LLM benchmarks on BERT and Llama 2 models. Our results show that we can achieve a 9\% model size reduction with minimal accuracy drops, which range from 4\%p (\%p refers to "percentage point," which refers to the absolute difference between two percentage numbers; 74\% -> 78\% = 4\%p increase) to 10\%p, depending on the difficulty of the benchmark, without any retraining to recover accuracy after decomposition. The results show that low-rank decomposition can be a promising direction for LLM-based applications that require real-time service at scale (e.g., AI agent and real-time coding assistant), where the latency is as important as the model accuracy.

==> backup/02_background_backup.tex <==
\section{Background and Motivation}
\label{sec:background}

%\HK{Add visualized information (table, figure, etc.) regarding the novelty; let's mention only published works (e.g., HEAT is arxiv only).}

We discuss backgrounds on the low-rank tensor decomposition and motivation toward our approach.


\begin{comment}
    
\subsection{Low-Rank Tensor Decomposition}
\label{subsec:lowrank_decomp}

We introduce tensor decomposition, specifically, Tucker Decomposition~\cite{tucker1996decomposition}, and how we apply it to compress LLMs.
% 
Tucker Decomposition decomposes a tensor into a smaller core tensor and a set of matrices equal to the order of the tensor.
% 
As shown in \autoref{fig:Tucker_Decomposition}, for a \(3^{rd}\) order tensor \(T \in \mathbb{R}^{n_1 \times n_2 \times n_3}\), Tucker Decomposition is computed as
% 
\[T \approx \Gamma\times_1U^{1}\times_2U^{2}\times_3U^{3} = K \]
% 
where \(\Gamma \in \mathbb{R}^{r_1 \times r_2 \times r_3}\), and \(U^1,~U^2,~U^3\) belong to \(\mathbb{R}^{r_1 \times n_1},\mathbb{R}^{r_2 \times n_2},\mathbb{R}^{r_3 \times n_3}\) respectively.
% 
Here, \(r_1,~r_2,~r_3\) represent the decomposition rank of tensor \(T\). The \(i\) mode product, \(i = 1,~2,~3\), of the core tensor \(\Gamma\) and the factor matrices \(U^{1,~2,~3}\) is defined as: 
% 
%\revision{$$Changed \times_1 to \times_2 and \times_3 below~and~fixed~other~typos$$}
% 
$$(\Gamma \times_1 U^1)(n_1,r_2,r_3) = \sum_{i_1=1}^{r_1} \Gamma(i_1,r_2,r_3)U^1(i_1,n_1)$$
% 
$$(\Gamma \times_2 U^2)(r_1,n_2,r_3) = \sum_{i_2=1}^{r_2} \Gamma(r_1,i_2,r_3)U^2(i_2,n_2)$$
% 
$$(\Gamma \times_3 U^3)(r_1,r_2,n_3) = \sum_{i_3=1}^{r_3} \Gamma(r_1,r_2,i_3)U^3(i_3,n_3)$$
% 
Since tensor decomposition approximates the original tensor, the error between the original tensor \(T\) and the reconstructed tensor \(K\) depends on the decomposition rank \(r_1,~r_2,~r_3\).
% 
For a given set of decomposition ranks, the relative error between the original and the reconstructed tensors satisfies
% 
$$\norm{T - (\Gamma\times_1U^{1}\times_2U^{2}\times_3U^{3})} \leq \epsilon \norm{T}$$
% 
where $\norm{T}$ is the \textit{norm} of $T$.
%
The goal of Tucker-decomposition is to minimize $\epsilon$, and it can be formulated as
% 
$$ \argmin_{\Gamma,U^1,U^2,U^3} \norm{T - (\Gamma\times_1U^{1}\times_2U^{2}\times_3U^{3})} $$
% 
\revision{
\input{algorithms/tucker_algorithm}
% 
\autoref{alg:tucker_algo} describes how we can compute the core tensor and the factor matrices using Higher-Order Orthogonal Iteration (HOOI).
% 
HOOI is an iterative algorithm to approximate the factor matrices, while it can be shown~\cite{de2000multilinear} that the optimal core tensor $\Gamma$ can be computed as
% 
$$\Gamma = T \times_1 (U^1)^T \times_2 (U^2)^T \times_3 (U^3)^T$$}
% 
Generally, a higher decomposition rank results in a better approximation. While the lower bound of \(r_1,~r_2,~r_3\) is \(1\), the upper bound is usually taken as \(r_i = n_i,~i = 1,2,3\) for a good approximation. In our experiments, we prune the decomposition rank \(r_1 = r_2 = r_3 \in [1, \min(n_1,n_2,n_3)]\). 
\end{comment}

\subsection{Computation in Language Models (LMs)}
\label{subsec:challenges_for_llms}

\insertFigure{ModelArchitecture}{The layer architecture of two recent language models: Bert~\cite{kenton2019bert} and Llama2~\cite{touvron2023llama}. Lin, BMM, and RMS refer to the linear layer, batched matrix multiplication, and root mean square, respectively.}

State-of-the-art language models~\cite{openai2023gpt4, touvron2023llama, anil2023gemini} today are mostly based on the Transformer~\cite{vaswani2017attention} architecture.
%
Although the original Transformer model was based on a full encoder-decoder structure, encoder-~\cite{kenton2019bert} and decoder-only~\cite{openai2023gpt4} models emerged as effective solutions with high task performance (e.g., accuracy).
%
Such models include multiple layers connected in a linear architecture, as illustrated in~\autoref{fig:DesignSpace} (a).


Although the layer architecture can differ depending on the model, as~\autoref{fig:ModelArchitecture} shows, the majority of operators, such as linear layer and batched matrix multiplication (BMM) are in common.
%
Among operators, linear operations (linear layer and BMM) account for approximately 75\% of the total execution time on CPUs~\cite{kim2023full}.
%
In addition, such linear operations involve a large number of parameters (e.g., 7 - 70 billion parameters for Llama2~\cite{touvron2023llama}), which results in large memory traffic and imposes a major challenge to efficient inference and generation.
%
A key concept that helps understand the large memory traffic challenge considering both computational throughput and memory bandwidth is the operational (or, arithmetic) intensity, which we discuss next.

%We further discuss such challenges comparing language models to convolutional neural network (CNN) next.

%
%Also, over \(80\%\) of the model parameters in BERT and over \(96\%\) of the model parameters in Llama-2 are present in the encoder and decoder layers respectively, and most of them are used for variants of matrix multiplications (e.g., linear and BMM).


%which makes them as the prime optimization target for efficient language model inference.

%Self-Attention (SA) is a key operator in Transformer-based language models. 
%
%In SA, the linear and batched matrix multiplication (BMM) accounts for the majority of the model's memory footprint.
%
%The multi-layer perceptron (MLP) layer in Llama and the intermediate/output layers in BERT are also based on matrix multiplication.
%

%
%\sout{Because of the relatively low dimensionality of such operators compared to convolutions, which reduces the data reuse across different dimensions and effectively lowers the number of computations for each data, the overall computation-to-model size ratio of language models is lower than that of convolutional neural networks, as shown in~\autoref{tab:arithmetic_intensity}.
%
%Therefore, Transformer-based language model workloads tend to be in the memory-bound region in the roof-line model~\cite{kim2023full}, which motivates optimizations focusing on the memory footprint and traffic.}
% 

\insertFigure{Roofline}{An example roofline that captures memory- and computation-bound workloads based on their arithmetic intensity. BW indicates bandwidth. Note that this is a high-level figure for illustrating concepts.}

%
%We first provide an overview of the operational intensity and roofline model~\cite{williams2009roofline} and use the concepts to discuss current challenges for language model optimization.

\subsection{Operational Intensity and Roofline Model}
%
Operational intensity refers to the number of operations per DRAM traffic bytes~\cite{williams2009roofline}, which quantifies the compute-to-off-chip-communication ratio for running a workload on a computer system.
%
Workloads with low arithmetic intensity implies more number of DRAM access than those with high arithmetic intensity, which tends to shift the system bottleneck to the memory bandwidth, not the computational throughput.
%
Such insights are visualized summarized in the roof-line model illustrated in~\autoref{fig:Roofline}.

The roofline model shows that the peak throughput of underlying hardware can be realized only if a workload has sufficiently large operational intensity.
%
If the operational intensity is low, the communication latency cannot be hidden within the computation latency when we apply computation-communication latency overlapping.
%
That is, the communication latency becomes visible beyond the computation latency, which leads to lower throughput than the underlying hardware's peak throughput.
%
In such cases, as illustrated in the memory-bound region in~\autoref{fig:Roofline}, the overall throughput is constrained by the memory bandwidth.
%
%The transition point distinguishing memory- and compute-bound region indicates the perfect balance between the data consumption rate by the compute units and the memory bandwidth.
%
Because operational intensity of a workload on hardware depends on software optimizations (e.g., if an inefficient compiler decides to flush data that will be reused soon after, the operational intensity may decrease), we use compute-to-model size for following discussions as the metric measuring the innate operational intensity characteristics of a workload.


\subsection{Challenges for Optimizing LM Performance}
\label{subsec:challenges_for_llms}

%\betterparagraph{Challenges for Fast and Efficient LM Inference}
%
To understand the challenges for optimizing language model inference, we analyze the compute-to-model size ratios of BERT-Base~\cite{kenton2019bert} model with 110 million parameters fine-tuned on SQuAD dataset~\cite{rajpurkar-etal-2016-squad}, and Llama-2-7B~\cite{touvron2023llama} model with 7 billion parameters.
%
We compare the analysis results against a widely adopted convolutional neural network (CNN) model, Resnet50~\cite{he2016deep} targeting classification tasks on ImageNet~\cite{deng2009imagenet} dataset.
%

~\autoref{tab:arithmetic_intensity} shows the analysis results assuming FP16 precision.
%
The analysis reveals two major challenges for language models compared to the CNN: (1) large scale in model size and number of operations and (2) low compute-to-model size ratio.
%
Firstly, we observe that the model sizes and the number of operations of two language models are 4.3 - 262.3 $\times$ and 1.4 - 103.5 $\times$ larger than ResNet50, respectively.
%
Such a large scale of language models motivates optimizations for computational performance.
%

However, we also observe a major roadblock that hinders computational performance optimization: low compute-to-model size ratio of language models, which is 35.4\% lower than ResNet50, on average.
%
Accordingly, previous works reported that language model inference worklaods are memory-bound \cite{kao2023flat, kim2023full}.
%
In decoder-only models popular today~\cite{touvron2023llama, openai2023gpt4}, such a characteristic originates from the heavy use of matrix-vector multiplication operations, which are known to have even lower arithmetic intensity than matrix-matrix multiplication\cite{kim2023full}.


Our analysis indicates that the correct approach to optimize the computational performance of language models needs to focus on reducing memory bandwidth requirement, not on-chip computational latency.
%
As a such optimization method, we explore low-rank decomposition of parameter tensors, which shifts the memory bandwidth/size overhead toward the computational overhead.
%
We discuss low-rank decomposition in the LM context next.


\begin{comment}
    
\revision{Compared to convolutional neural networks (CNNs) that contain CONV2D, matrix multiplication has a lower data reuse opportunity in general\cite{kao2023flat},\cite{kim2023full}.
% 
In addition, decoder-only models, which are popular today (e.g., GPT and LLama2), involve heavy matrix-vector multiplication operations, which are known to have even lower arithmetic intensity than matrix-matrix multiplication\cite{kim2023full}.
% 
Because the roof line performance (or the best achievable performance) is proportional to the number of operations divided by the number of required memory accesses for the operations\cite{kao2023flat}, the Transformer based language models tend to be in the memory-bound region in the roof line model~\cite{kim2023full}.
%
Further,~\autoref{tab:arithmetic_intensity} compares the ratio of the number of computations and the model's size.
% 
It clearly shows that language models have a lower compute-to-model-size ratio than CNNs.
% 
This motivates optimizations that focus on memory footprint and traffic.
}

\end{comment}


\subsection{Tucker Decomposition (TKD) for Language Models}
\label{subsec:bg_tucker_decomposition}

Low-rank decomposition (LD) refers to techniques that factorize tensors into multiple smaller tensors, matrices, or vectors and prune unimportant factors in the decomposed space.
%
That is, LD can be utilized for compressing LMs with proper choice of the pruning factor. 
%
Popular LD approaches include Canonical Polyadic Decomposition (CPD)\cite{Harshman1970FoundationsOT}, Tensor-Train Decomposition (TTD) \cite{GNNTensorTrain, nips2020tensortrain}, and Tucker Decomposition (TKD) \cite{D-Tucker}.
%

\betterparagraph{Motivation toward TKD} 
\sout{
TTD is mainly adpoted for quantum simulation(\TODO{Add citation}) and is not popular for decomposing deep learning models (\TODO{Why?})(\FT{not sure about the claim. Reference:}\cite{nips2020tensortrain}).
}
\revision{a}
%
CPD is reported to result in unstable convergence~\cite{doi:10.1137/06066518X, Lebedev2014SpeedingupCN}, which imposes a major challenge to the model training process.
%

Compared to CPD, TKD is more friendly for training process due to its capability of capturing complex data patterns using multi-dimensional factors~\cite{tucker-cp-comp}.
%
Also, TKD involves deterministic tensor dimensions directly controlled by the choice of a parameter, pruned rank.
%
Therefore, we focus on TKD as our methodology and discuss technical details of TKD next.

%Between CPD and TKD, we focus on TKD because of the following reasons: (1) CPD's Unstable convergence\cite{doi:10.1137/06066518X, Lebedev2014SpeedingupCN}, (2) TKD's deterministic tensor dimensions directly controlled by the hyperparameters, and (3) TKD's multi-dimensional factors allowing to capture complex data patterns\cite{tucker-cp-comp}(\FT{Added citation}).
% 
%Firstly, CPD may have unstable convergence as noted by De Silva and Lim\cite{doi:10.1137/06066518X} and Lebedev et al.,\cite{Lebedev2014SpeedingupCN}.
% 
%Secondly, because Tucker decomposition produces only a fixed number of factor matrices, it is easier to use it for model compression compared to CPD, in which the number of factor matrices depends on the pruned rank.
%
%Lastly, Tucker decomposition is also favorable because it allows for better control of the decomposition rank and can capture complex data patterns hidden in the intrinsic ranks of the input tensor because of the core tensor.}
% 
%\\\
%}

%increasing their operational intensity by reducing the memory traffic and shifting that overhead to the computation.
%
%Such an optimization is a valid optimization since LMs are memory-bound, as discussed in~\autoref{subsec:challenges_for_llms}.

\betterparagraph{TKD Formulation}
TKD decomposes a tensor into a smaller core tensor and a set of matrices equal to the order of the tensor, as illustrated in~\autoref{fig:Tucker_Decomposition}.
% 
For a \(3^{rd}\) order tensor \(T \in \mathbb{R}^{n_1 \times n_2 \times n_3}\), Tucker Decomposition can be summarized as the following:
% 
\[T \approx \Gamma\times_1U^{1}\times_2U^{2}\times_3U^{3} = K \]
% 
where \(\Gamma \in \mathbb{R}^{r_1 \times r_2 \times r_3}\) and $U^i \in \mathbb{R}^{r_i \times n_i}$ for $i=1,2,3$.
%\(U^1,~U^2,~U^3\) belong to \(\mathbb{R}^{r_1 \times n_1},\mathbb{R}^{r_2 \times n_2},\mathbb{R}^{r_3 \times n_3}\) respectively.
% 

In the formula, \(r_1,~r_2,~r_3\) represent the decomposition ranks of a 3D tensor \(T\) (i.e., the rank after decomposition and pruning), and the tensor K represent the approximation of the 3D tensor $T$ obtained by the decomposition.
%
%The \(i\)-mode product for \(i = 1,~2,~3\) of the core tensor \(\Gamma\) and the factor matrices \(U^{1,~2,~3}\) is defined as: 
% 
%\revision{$$Changed \times_1 to \times_2 and \times_3 below~and~fixed~other~typos$$}
% 

\betterparagraph{$i$-mode Product in TKD}
The \(i\)-mode product refers to the multiplication of core tensor with the i-th factor matrix, which is performed in the process of reconstructing the original tensor dimension.
%
For \(i = 1,~2,~3\) of the core tensor \(\Gamma\) and the factor matrices \(U^{1,~2,~3}\) is defined as: 

$$(\Gamma \times_1 U^1)(n_1,r_2,r_3) = \sum_{i_1=1}^{r_1} \Gamma(i_1,r_2,r_3)U^1(i_1,n_1)$$
% 
$$(\Gamma \times_2 U^2)(r_1,n_2,r_3) = \sum_{i_2=1}^{r_2} \Gamma(r_1,i_2,r_3)U^2(i_2,n_2)$$
% 
$$(\Gamma \times_3 U^3)(r_1,r_2,n_3) = \sum_{i_3=1}^{r_3} \Gamma(r_1,r_2,i_3)U^3(i_3,n_3)$$

\betterparagraph{TKD Objective Function}
Since tensor decomposition approximates the original tensor, the error between the original tensor \(T\) and the reconstructed tensor \(K\) depends on the decomposition rank \(r_1,~r_2,~r_3\).
% 
For a given set of decomposition ranks, the relative error between the original and the reconstructed tensors satisfies
% 
$$\norm{T - (\Gamma\times_1U^{1}\times_2U^{2}\times_3U^{3})} \leq \epsilon \norm{T}$$
% 
where $\norm{T}$ is the \textit{norm} of $T$.
%
The goal of Tucker-decomposition is to minimize $\epsilon$, and it can be formulated as
% 
$$ \argmin_{\Gamma,U^1,U^2,U^3} \norm{T - (\Gamma\times_1U^{1}\times_2U^{2}\times_3U^{3})} $$
% 
\input{algorithms/tucker_algorithm}

\revision{
% 
\betterparagraph{TKD Algorithm} \autoref{alg:tucker_algo} describes Higher-Order Orthogonal Iteration (HOOI), an iterative algorithm computing a core tensor and factor matrices of a tensor$T$~\cite{de2000multilinear}.
%
The algorithm keeps performing SVD for each factor matrix until the convergence criteria are met.
%
%Following the algorithm, the optimal core tensor $\Gamma$ can be computed as follows:
% 
%$$\Gamma = T \times_1 (U^1)^T \times_2 (U^2)^T \times_3 (U^3)^T$$}
% 
Generally, a higher decomposition rank results in a better approximation.
%
While the lower bound of \(r_1,~r_2,~r_3\) is \(1\), the upper bound is usually taken as \(r_i = n_i,~i = 1,2,3\) for a good approximation. In our experiments, we prune the decomposition rank \(r_1 = r_2 = r_3 \in [1, \min(n_1,n_2,n_3)]\). 
}


\begin{comment}
TKD can be viewed as a generalized case of Singular Value Decomposition (SVD)~\cite{zare2018extension} with pruned low-rank factor matrices to approximate the original matrix.
%
For example, second-order TKD can be computed as multiplication of core and factor matrices:
\revision{
$$T(n_1,n_2) \approx (U^1(PR,n_1))^T \times \Gamma(PR,PR) \times U^2(PR,n_2) = K$$
}
where $PR$ is the $pruned$ $rank$, which refers to the number of ranks chosen after decomposition (smaller than the original rank).

As shown in \autoref{fig:DesignSpace}(c), a 2D tensor \revision{\(W_v \, \in \, R^{H \times W}\)} can be approximated by the product of a core tensor and two factor tensors with pruned ranks.
%
The core tensor \revision{\(B \, \in \, R^{PR \times PR}\)}, where \(PR\) is the pruned rank, while the factor matrices \(A \, \in \, R^{H \times PR}\) and \revision{\(C \, \in \, R^{PR \times W}\)}.
% 
\end{comment}


\betterparagraph{Model Compression using TKD}
To effectively compress the model, the ranks after low-rank pruning, pruned rank (PR), needs to be carefully selected. 
%
We formulate the maximum PR that makes the resulting model smaller than the original model.
%
First, we compute the number of parameters before and after the decomposition and the compression ratio using them.
%
$$\# ~parameters~before~decomposition = H \times W$$
$$\#~parameters~after~decomposition = H \times PR + PR \times PR + PR \times W$$
$$Compression~Ratio = \frac{H \times W}{H \times PR + PR \times PR + PR \times W}$$
%
The formula indicates that the smaller the PR is (preferably, PR << min(H,W)), the higher the compression ratio is.
%

%\betterparagraph{Choice of PR for Compression}
To achieve compression effect, the compression ratio needs to be larger than 1, which can be represented as follows:
%
$$Compression~Ratio > 1$$
$$\frac{H \times W}{H \times PR + PR \times PR + PR \times W} > 1$$
%
Rearranging terms in the above inequality, we obtain the following: $$PR^2 + (H + W) \times PR - H \times W < 0$$
%
Solving the above quadratic inequality for PR, the results indicate the upper-bound of the pruned rank that can compress the model, which is presented as follows:
%
$$PR < (\frac{\sqrt{(H+W)^2 + 4\times H\times W} - (H + W)}{2})$$
%
Note that the inequality above indicates the upper-bound value of PR for compression.
%
As discussed, lower PR leads to better compression ratio.
%
Therefore, minimizing PR while maintaining the model performance is one of the key optimizations needed for TKD.

%If \(PR \ll \min(H,~W)\), or \(PR < (\frac{\sqrt{(H+W)^2 + 4\times H\times W} - (H + W)}{2})\) \revision{(equation \ref{eq:pr})} more specifically, the total number of parameters reduce because of decomposition, and the compression ratio can be computed as:

% 

%\betterparagraph{Canonical Polyadic (CP) Vs Tucker decomposition} CP decomposition (CPD)\cite{Harshman1970FoundationsOT} is another methodology for tensor decomposition.
% 
%It achieves more compression than Tucker Decomposition (TKD) because of the absence of a core tensor.
% 
%However, CPD may have instability issues for low-rank decompositions as reported by De Silva and Lim\cite{doi:10.1137/06066518X} and Lebedev et al.,\cite{Lebedev2014SpeedingupCN}.
% 
%On the other hand, Tucker decomposition offers higher convergence stability and ease of implementation as the input tensor is split into just three factors, whereas in the case of CPD, the number of factor matrices depends on the pruned rank. 
%


%and determine if we can maintain accuracy similar to the original model.


%inspired us to investigate whether the key parameters of the original model during inference generally also occupy a low intrinsic dimension.
% 
%If t, we could decompose matrices to smaller sizes while maintaining accuracy comparable to the larger model.
% 
%Specifically, LoRA utilizes additional low-rank decomposed tensors to update (fine-tune) the model's parameters.
% 
%In contrast, our approach decomposes the model's parameter tensors themselves to achieve a more concise representation and determine if we can maintain accuracy similar to the original model.

\subsection{Problem Statement}
\label{subsec:problem_statement}

%In this section, we highlighted (1) the motivation toward computational performance optimization of LMs from their large scale and (2) challenges for optimization from their low operational intensity.
%
%As discussed in~\autoref{subsec:challenges_for_llms}, LMs are memory-bound, which motivates us to explore optimization techniques focusing on enhancing the operational intensity by reducing memory bandwidth requirement.
%
%Among potential approaches, we focus on TKD since its friendly characteristics for training and performance optimization, as discussed in~\autoref{subsec:bg_tucker_decomposition}.
%

As discussed in~\autoref{subsec:challenges_for_llms}, LMs are memory-bound, which motivates us to explore optimization techniques that enhance the operational intensity by reducing memory bandwidth requirement.
%
TKD with rank-pruning is a promising approach for that as discussed in~\autoref{subsec:bg_tucker_decomposition}, but the approach involves a major trade-off between the model performance (e.g., accuracy) and computational performance (e.g., latency) due to the nature of rank pruning, which is not well-explored yet.
%

Therefore, to shed a light into the trade-off, we aim to (1) \textit{profile the accuracy-computational performance trade-off space of TKD on recent LMs and report the insights from the results}.
%
Also, to enable systematic trade-off space exploration, we aim to (2) \textit{formulate the TKD design choices and space}.
%
Finally, we aim to (3) \textit{identify effective design choices of TKD}, which can be useful insights for effective TKD trade-off space exploration.
 


\begin{comment}
    
Challenge: Low-arithmetic intensity (Memory-bound) -> To optimize LLM, we need to optimize for memory usage, rather than computational performance.

\revision{1. Moving memory overhead to computational overhead via TKD}
Roof-line model



\revision{2. Compression by pruned rank}
Some prior works demonstrate that low-rank decomposition can be effective in specific problems within LLMs.
% 
Among these, LoRA \cite{hu2022lora} represents a state-of-the-art approach that employs low-rank decomposed matrices for fine-tuning.
% 
LoRA builds on the earlier idea \cite{intrinsic_dim, aghajanyan2020intrinsic} that the number and distribution of parameters adjusted during fine-tuning for a specific task reside within a low intrinsic dimension.
% 
This inspired us to investigate whether the key parameters of the original model during inference generally occupy a low intrinsic dimension.
% 
If so, we could decompose matrices to smaller sizes while maintaining accuracy comparable to the larger model.
% 
Specifically, LoRA utilizes additional low-rank decomposed tensors to update (fine-tune) the model's parameters.
% 
In contrast, our approach decomposes the model's parameter tensors themselves to achieve a more concise representation and determine if we can maintain accuracy similar to the original model.

\end{comment}


==> backup/03_Methodology.tex <==
%
We use a $2^{nd}$ order weight tensor ($W_{orig}$) as an example to discuss the computation order we select.
%
In matrix multiplication notation, the decomposition of $W_{orig}$ can be represented as follows:
$$
W_{orig} \approx W_{apprx} = F_{1} \times \Gamma \times F_{2}
$$
%
Assume that $W_{orig}$ is a $d1 \times d2$ matrix, and pruned rank is $PR$.
%
Then, the dimensions of $F_{1}$, $F_{2}$, and $\Gamma$ are ($d1 \times PR$, $PR \times d2$, and $PR \times PR$.
%
Applying the approximated weight to a linear layer with input $I$ and output $O$ tensors, we obtain the following:
\begin{align*}
O \approx I \times W_{apprx} &= I \times (F_{1} \times \Gamma \times F_{2}) \\
&= I \times F_{1} \times \Gamma \times F_{2}
\end{align*}
%
The first line reconstruct weight and run the original linear layer, and the second line gradually compute the final results without reconstructing the original weight.
%
Letting the input tensor $I$ dimension is $(len, d1)$, the number of FLOPs for the first approach (reconstruct weight and run linear layer) can be computed as follows:
%
\begin{align*}   
FLOPs_{reconstruction} &= d1 \times PR \times PR + d1 \times PR \times d2 \\ 
FLOPs_{Linear} &= len \times d1 \times d2 \\ 
FLOPs_{approach1} &= FLOPs_{reconstruction} + FLOPs_{Linear}
\end{align*}
%
For the second approach (gradually compute the final results), the number of FLOPs can be computed as follows:
\begin{align*}  
FLOPS_{approach2} &= len \times d1 \times PR + len \times PR\times PR + len \times PR \times d2
\end{align*}
%
In LLM settings 

For LLama-2-7B (d1 = d2 = 4096), small pruned rank (e.g., 1), and the sequence length of 1000,
$$
FLOPs_{approach1} = 4096 \times 1 \times 1 + 4096 \times 1 \times 4096 + 1000 \times 4096 \times 4096 = 
$$























\begin{comment}    
That is, for $2^{nd}$ order weight matrix as an example, we select to compute the following matrix multiplication in order from left to right (last line), instead of first reconstructing weight (first line)
\begin{align*}
O \approx I \times W_{apprx} &= I \times (F_{1} \times \Gamma \times F_{2}) \\
&= I \times F_{1} \times \Gamma \times F_{2}\\
(O: Output,\quad &I: Input, \quad F_{i}: Factor \ i, \quad \Gamma: core)
\end{align*}
%
For example, a linear layer with the input/output dimension of 4096 in Llama-2-7B with PR of 1, the second approach (gradual) reduces 99.9\% of FLOPs compared to the first approach (reconstruction). 
%
As we reduce the total number of parameters via TKD with a small pruned rank and the FLOPs with computation ordering, the overall number of computations and memory usage decrease, which improves the inference latency and energy.
%
However, the design space of low-rank decomposition is huge, so we need a formal methodology to perform low-rank decomposition.
\end{comment}

==> backup/04_CaseStudy.tex <==

%
%If we classify common-sense reasoning benchmarks based on inference accuracy, we can consider benchmarks like ARC Easy and WinoGrande simpler than ARC Challenge, HellaSwag, MMLU, and GSM8K, as they have higher inference accuracy.
% 
%For such relatively easy benchmarks, the decline in accuracy is smaller as the decomposition percentage increases compared to more challenging benchmarks.

% 
% For easier common-sense reasoning benchmarks like ARC Easy and WinoGrande, where model accuracy is high to start with, the degradation of accuracy with an increase in decomposition percentage is less compared to more difficult benchmarks like ARC Challenge, HellaSwag, MMLU, and GSM8k.
% 
% For ARC Easy, every percentage of parameter reduction results in a percentage drop in accuracy, or about \(7.4\) points decrease in absolute accuracy.
